Investigating Explainability of Generative AI for Code through Scenario-based Design

What does it mean for a generative AI model to be explainable? The emergent discipline of explainable AI (XAI) has made great strides in helping people understand discriminative models. Less attention has been paid to generative models that produce artifacts, rather than decisions, as output. Meanwhile, generative AI (GenAI) technologies are maturing and being applied to application domains such as software engineering. Using scenario-based design and question-driven XAI design approaches, we explore users' explainability needs for GenAI in three software engineering use cases: natural language to code, code translation, and code auto-completion. We conducted 9 workshops with 43 software engineers in which real examples from state-of-the-art generative AI models were used to elicit users' explainability needs. Drawing from prior work, we also propose 4 types of XAI features for GenAI for code and gathered additional design ideas from participants. Our work explores explainability needs for GenAI for code and demonstrates how human-centered approaches can drive the technical development of XAI in novel domains.

==> content/arxiv.tex <==
% ---- abstract ------
There have been many studies about the explainability of discriminative AI models (XAI), but the explainability of generative AI models is under-investigated. 
Most recently, generative AI models for code, aiming to mimic human-written code and assist software engineers during the development, has raised great attention in the AI community. 
However, what kinds of explainability needs engineers have in terms of generative AI models for code remains an open problem.
We conducted 9 scenario-based workshops to elicit both critiques and design concepts from 43 software engineers. 
These workshops span across 3 use cases of generative AI models for code, including code autocompletion, natural language to code, and code translation. 
By doing so, we aim to understand the explainability needs of software engineers, identify gaps between the current XAI frameworks for discriminative AI models and the real needs of generative AI models for code and further inform the AI community to develop products that address the XAI pain points. 
To achieve this goal, we designed user journeys in each workshop with real examples from the state-of-the-art generative AI models for code to ground the brainstorming. Inspired by the existing work of XAI needs, we designed 3 UX prototypes that address XAI features to spike the discussion and get user feedback to identify the design needs.
Our work sheds light on the design space of explainability of generative AI for code and identifies opportunities for future XAI work. 
We design 4 explainability features in the context of generative models for code and get user feedbacks for refinement and improvement.
We also connect the XAI needs from our study with state-of-the-art technologies to identify opportunities and challenges.


%% JW alternate abstract
\textbf{JW alternate abstract:}
What does it mean for a generative AI model to be \emph{explainable}? The emergent discipline of explainable AI (XAI) has made significant progress in developing both technical and non-technical means for explaining the operation, the outputs, and the use of discriminative ML models. Less attention has been paid to the explainability needs of people who work with generative ML models: those that learn to produce artifacts, rather than decision boundaries. Using a scenario-based design approach, we explore explainability needs for generative ML models in the context of software engineering. Many recent advances in the ML community have shown how generative models, including large language models not specifically trained on code, can produce working code from natural language descriptions, can translate code from one language to another, and can even autocomplete code from a comment and a method signature. We conducted {\color{red}9} workshops with {\color{red}N} software engineers focused around each of these three use cases, using real examples from state-of-the-art generative AI models for code as a basis for brainstorming explainability needs. We also employed multiple provocations to elicit both technical and non-technical explainability needs. Through a {\color{red}thematic analysis}, we identified {\color{red}X} categories of explainability needs, {\color{red}X} of which have not currently been addressed by prior XAI research, such as {\color{red}X}, {\color{red}Y}, and {\color{red}Z}. Our work pushes the boundaries of explainable AI to include generative models, and identifying new and unmet explainability needs.


\textbf{Vera built on Justin's}
What does it mean for a generative AI to be \emph{explainable}? The emergent discipline of explainable AI (XAI) has produced rich means to help people understand discriminative ML models. Less attention has been paid to generative ML models, which lean to produce plausible contents or artifacts. Using scenario-based design, we explore explainability needs for generative ML models in the context of software engineering. Recent advances in ML have shown that generative models can be used to produce code from natural language descriptions, translate code from one language to another, and autocomplete code. We conducted {\color{red}9} workshops with {\color{red}N} software engineers focused on these use cases, using scenario-based design combined with output from state-of-the-art generative models to explore users' explainability needs. We also propose 4 types of XAI features to elicit design ideas from participants. Our work lays out the space of explainability needs and suggests XAI solutions to support users of generative AI for code. We also push the boundaries of XAI to include generative models, and contribute a human-centered approach to drive technical development of XAI in novel domains.  

\textbf{jiao final}:
What does it mean for a generative AI model to be \emph{explainable}? The emergent discipline of explainable AI (XAI) has made significant progress in understanding discriminative ML models. Less attention has been paid to generative ML. Using a scenario-based design approach, we explore explainability needs of generative ML models for software engineering. Recent advances have shown how generative models can produce code from natural language, translate code and even autocomplete code. We conducted 9 workshops with 43 software engineers focused on these three use cases, using real examples from state-of-the-art generative AI models. We also propose 4 XAI features to elicit design ideas from participants. Our work lays out the space of explainability needs and suggests XAI solutions to support users of generative AI for code. We push boundaries of XAI to include generative models and contribute a human-centered approach to drive the technical development of XAI in novel domains.

\textbf{Justin final v2}:
What does it mean for a generative AI model to be \emph{explainable}? The emergent discipline of explainable AI (XAI) has made enormous strides in helping people understand discriminative models. Less attention has been paid to generative models that produce \emph{artifacts}, rather than \emph{decisions}, as output. Using a scenario-based design approach, we explore explainability needs for generative models in three software engineering use cases: natural language to code, code translation, and code autocompletion. We conducted 9 workshops with 43 software engineers in which real examples from state-of-the-art generative AI models were used to elicit explainability needs. Our work identified {\color{red}N} new categories of explainability needs for generative code models, and demonstrates how human-centered approaches can drive the technical development of XAI in novel domains.

% ------------------ end of abstract ---------------------


% ------------------ preliminary result ---------------------
\subsection{Preliminary Results}
As of this writing, we have conducted 8 workshops with 40 software engineers within IBM. In a preliminary analysis, we have started grouping the comments and questions raised in these workshops in 3 broad categories: questions about model, questions about the code produced by the model, and questions about human-AI collaboration. Some of the specific kinds of questions asked about the model and the code it produces include:

\begin{itemize}
    \item \emph{Model Efficiency}. Participants wondered about the  time efficiency of the model (i.e. how long it takes to run inference), as well as how it compares with other competitor tools. They also wanted to know about the models' performance evaluation and what metrics it was evaluated on (e.g., correctness, time and space complexity).
    \item \emph{Model Interpretability}. Participants wanted to understand the mechanisms of how the model worked and how it was trained (e.g., ''how exactly does it generate code? is it pulling from sites or using GANs to generate new code'', ''brief summary on algorithm behind AI''). In addition, they wanted to understand whether the model actually learns coding logic or if it just captures lexical information.
    \item \emph{Model Uncertainty}. Participants desired to understand multiple possibilities considered by the model, rather than treating the model as a box that takes in a single input and produces a single output. For example, in the code translation use case, our participants mentioned, ''Are there multiple translations available? If so, how can they be shuffled through/accessed?'' 
    \item \emph{Platform}. Participants wanted to know about the model's dependencies, hosting requirements, and how to deploy the system (e.g., hardware requirements such as NVIDIA GPUs, how to deploy the system in a live production environment, supported operating systems, and supported IDEs.)
    \item \emph{Transparency}. Participants were eager to know what the models were capable of doing, as well as what their limitations were, such as known pitfalls or degenerate input cases.  
    \item \emph{Safety}. Participants were concerned about privacy and data use policies, such as the use of user-generated content to train the model and source code licenses. Some participants had heated discussions of the legal issues surrounding the model's use and production of intellectual property. Participants asked questions including, ''Can I use the AI in closed source project?'' ''How was it trained and how does it respect the licenses of the code it trained on?'' and ''Where will the generated code be stored?'' 
    \item \emph{Green AI}. AI models are known for being computationally expensive to train and use. Participants were concerned about how using the model would affect energy usage (e.g. CPU/GPU usage, battery drain).
\end{itemize}

Participants emphasized the need to understand the code generated by the model. Such explainability of code includes its efficiency, correctness, ability to handle edge cases, and coding style. This explainability of code seemed very important to participants in order for them to effectively work with the model.

% ------ end of preliminary result ---------------------



==> tables/question-bank-old.tex <==
\begin{table}[]
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}l|l|l|l@{}}
\toprule
%\textbf{Input} & \begin{tabular}[c]{@{}l@{}}- What types of data types, data structures, algorithms, etc., \\   does the AI know/understand?\\ - How specific does the input need to be to get good output?\\ - What kind of inputs can the AI reasonably generate code from?\\ - Numbers of words or detailing required?\end{tabular}

%& \textbf{Output} & \begin{tabular}[c]{@{}l@{}}- Will this produce idiomatic Python code, or an 1:1 translation?\\ - Will there be automated tests generated?\\ - Can the model generated code that does error/exception \\    handling correctly?\\ - How confident are you about the solution? \\ - IP protection for AI generated products \\\end{tabular} \\ \midrule
\textbf{How (global)} & \begin{tabular}[c]{@{}l@{}}- Will the translation consider taking advantages of Python language?\\ - Looking to create guidelines for how to use the model effectively?\\ - How exactly does it generate code? is it pulling from sites or using GANs?\\ - How close it can comprehend my thought process or my language?\end{tabular} & \textbf{Performance} & \begin{tabular}[c]{@{}l@{}}- How correct is the translation guaranteed to be?\\ - How accurate is the model?\\ - Is this the most efficient (CPU, memory) solution to this problem?\\ - efficiency and optimization when it comes to real world\end{tabular} \\ \midrule
\textbf{How to} & \begin{tabular}[c]{@{}l@{}}- How can I get AI to write efficient code?\\ - Can we make clarification to the code after the AI system has written code?\\ - How exact one has to to be in writing statement so AI can understand?\\ - How can I optimize for one over another?\end{tabular} & \textbf{Customization} & \begin{tabular}[c]{@{}l@{}}- Can I select a preference for datatypes/packages used?\\ - Can I tune the translation?\\ - Is there a setting for the AI where he can turn off/on?\\ - Any specific regional settings that you want to apply?\end{tabular} \\ \midrule
\textbf{Why (local)} & \begin{tabular}[c]{@{}l@{}}- Alex wonders how AI knows what is a prime number?\\ - How AI is recognizing the function from comments?\\ - Why did AI think that code satisfied the requirement. \\    Can it link to relevant explanations?\\ - Interesting that 4th attempt with the least programming thinking \\   gave good result\end{tabular} & \textbf{Data} & \begin{tabular}[c]{@{}l@{}}- What data was this trained on?\\ - What code was the AI trained on? Where does it pull from?\\ - Where is the code coming from? Some websites?\\ - What kind of training set was the AI built with?\end{tabular} \\ \midrule
\textbf{\begin{tabular}[c]{@{}l@{}}System \\ Requirement\end{tabular}} & \begin{tabular}[c]{@{}l@{}}- Can I use it in closed source project?\\ - Does it work on Apple GPUs or only Nvidia?\\ - Can I use it in my development environment?\\ - Does the requirement change?\end{tabular} & \textbf{Others} & \begin{tabular}[c]{@{}l@{}}\textbf{What if}:              - What about overflow?\\                             - What to return if input invalid?\\ ----------------------------------------------------------------------------------\\ \textbf{System Impact}:    - How does the model affect CPU/GPU usage \\                                 or battery life of Alex's laptop?\\ ----------------------------------------------------------------------------------\\ \textbf{Why not}:              - Why doesn't my given inputs work?\end{tabular} \\ \bottomrule
\end{tabular}
}
\caption{XAI question bank for generative AI for code. The table is ranked by the number of questions under each code horizontally (i.e., Input, Output, How (global)...), which indicates the importance of each category from the users' point of view.}
\label{tab:question-bank}
\end{table}

% \begin{table}[htp]
%     \centering
%     \begin{tabularx}{\linewidth}{p{2cm}XXp{1.6cm}}
% \end{table}

% \begin{longtable}{p{.15\linewidth}p{.30\linewidth}p{.30\linewidth}p{.15\linewidth}}
%     \toprule
%     \textbf{Category} & \textbf{Description} & \textbf{Exemplar Questions} & \textbf{Technical\allowbreak Approaches} \\
%     \midrule
%     \endfirsthead
%     \toprule
%     \textbf{Category} & \textbf{Description} & \textbf{Exemplar Questions} & \textbf{Technical\allowbreak Approaches} \\
%     \midrule
%     \endhead

\begin{table}[htp]
    \small
    \centering
    \begin{tabularx}{\linewidth}{XXp{1.6cm}}
        \toprule
        \textbf{Category \& Description} & \textbf{Exemplar Questions} & \textbf{Technical\allowbreak Approaches} \\
        \midrule
        \textbf{Input}. Questions about the kinds of inputs taken by the model, the kinds of inputs for which the model produces good results\sout{, and how changes in input affect the quality of the model's output}. & What kind of inputs can the model reasonably generate code from? How specific or descriptive does my input need to be to get good output? What kinds of problems can the model write function definitions for? \sout{Can I give hints to improve the model's output? Do I need to learn certain tricks in how to specify my problem to get good output?} \\
        \midrule
        \textbf{Output}. Questions about the quality of the output, its equivalency to the input, the confidence of the model, and alternative options produced by the model. & Will the translated code have the same complexity as the original? Will the variable names be the same? What other code options did the AI generate? How confident are you about the solution? \\
        \midrule
        \textbf{Performance}. Questions about the runtime performance of the model: how long it will take to produce output, and how its performance is affected by the size of input. & How much time will it take to translate the code? How will be the performance of the code for larger inputs? \\
        \midrule
        \textbf{How (global)}. Questions about how the model operates. & Python is dynamically typed, Java is static, how does it enforce these typing rules? How exactly does it generate code? Does the AI optimize for big O (either in time or space)? Can this AI use design patterns? \\
        \midrule
        \textbf{Why, Why not}. Questions about why the model produced a given output or why a given input failed to produce the desired output. & Why did AI think that code satisfied the requirement, can it link to relevant explanations, API documentation, use cases, etc.? Why didn't my given inputs work? \\
        \midrule
        \textbf{What if}. {\color{red}I'm not seeing any good what if questions} & \\
        \midrule
        \textbf{How to be that, how to still be this}. Questions about how to control the quality or characteristics of the output and how changes in input affect the quality of the model's output. & {\color{red}All of the questions about controlling output should be considered ``how to be that'' but they are currently classified as Input. So I left those above and just struck them out.} Can I give hints to improve the model's output? Do I need to learn certain tricks in how to specify my problem to get good output? \\
        \midrule
        \textbf{System Requirements \& Impact$^\dagger$}. Questions about the system requirements to use the model and appropriate uses of the model's output. & What are the hardware requirements for using the model? What is the energy consumption of using the model? Can I use the model's output in a closed source project? \\
        \midrule
        \textbf{Customization$^\dagger$}. Questions about tuning the model or specifying preferences that govern the model's output. & Can I tune the translation? Can I select a preference for datatypes/packages used? Can I set specific regional settings? \\
        \midrule
        \textbf{Data$^\dagger$}. Questions about the provenance of the data on which the model was trained. & What data was this trained on? What kind of training set was the AI built with? \\
        \midrule
        \textbf{Limitations$^\dagger$}. Questions about the limitations of the model's capabilities. & What limits are there to the model's function? What scenarios does it cover? What are the limits on the algorithms the AI can generate? \\
        \bottomrule
    \end{tabularx}
    \caption{Categories of questions that emerged from our workshops. We classified questions using the XAI question framework of \citet{liao2020questioning}; categories marked with a dagger ($\dagger$) represent new categories of questions that emerged due to the generative AI context. For each question category, we provide an overall description of the kinds of questions raised by participants, as well as a few exemplar examples in participants' own words. For some categories of questions, we also provide references to technical approaches that may be used to answer questions in those categories. Categories with no listed technical approaches represent open areas for future machine learning and explainable AI research. \vera{from JW: should we give counts/percentages for how many times questions occurred in each category? possibly not because some of these categories are small. also, was there consensus in coding? i'm seeing inconsistencies, like questions about controlling output are appearing in both How (global) and Input.}}
    \label{tab:question-bank-v2}
\end{table}
